An Approach to Technical AGI Safety and Security

Artificial General Intelligence (AGI) promises transformative benefits but also presents significant risks. We develop an approach to address the risk of harms consequential enough to significantly harm humanity. We identify four areas of risk: misuse, misalignment, mistakes, and structural risks. Of these, we focus on technical approaches to misuse and misalignment. For misuse, our strategy aims to prevent threat actors from accessing dangerous capabilities, by proactively identifying dangerous capabilities, and implementing robust security, access restrictions, monitoring, and model safety mitigations. To address misalignment, we outline two lines of defense. First, model-level mitigations such as amplified oversight and robust training can help to build an aligned model. Second, system-level security measures such as monitoring and access control can mitigate harm even if the model is misaligned. Techniques from interpretability, uncertainty estimation, and safer design patterns can enhance the effectiveness of these mitigations. Finally, we briefly outline how these ingredients could be combined to produce safety cases for AGI systems.

==> scratch/writing-notes.tex <==
Still need to review:

- \textbf{AI capabilities can be significantly improved without expensive retraining} [CITATION]
- Vlad's doc: See https://docs.google.com/document/d/1MrIxXsfI2ZnL-nBWPscPxmFbZfu3HveneEmlpLnXXGY/edit?tab=t.i58x6bkji6iv for more on this.
- Vlad's claim: I'm a bit nervous about making this claim (only 2 very big jumps) given the lit review I did isn't fully exhaustive. I'd give maybe 20\% that you could find another task like this if you really looked?

